Information Theoretic Regret Bounds for Online Nonlinear Control

This work studies the problem of sequential control in an unknown, nonlinear dynamical system, where we model the underlying system dynamics as an unknown function in a known Reproducing Kernel Hilbert Space. This framework yields a general setting that permits discrete and continuous control inputs as well as non-smooth, non-differentiable dynamics. Our main result, the Lower Confidence-based Continuous Control ($LC^3$) algorithm, enjoys a near-optimal $O(\sqrt{T})$ regret bound against the optimal controller in episodic settings, where $T$ is the number of episodes. The bound has no explicit dependence on dimension of the system dynamics, which could be infinite, but instead only depends on information theoretic quantities. We empirically show its application to a number of nonlinear control tasks and demonstrate the benefit of exploration for learning model dynamics.

==> setting.tex <==

\section{Setting}

\sk{what do we actually need here? }

\iffalse
Consider a control problem with nonlinear system
dynamics described by:
\begin{align}
  x_{h+1}=f(x_h,u_h) + \epsilon_h, \textrm{ where } \epsilon_h \sim
  \mathcal{N}(0,\sigma^2 I) \label{eq: dynamicalsystem}
\end{align}
where the state $x_h\in\mathcal{X} $ with $\mathcal{X}=\R^{d_\mathcal{X}}$; the control $u_h \in\mathcal{U}$
with $\mathcal{U}$ being an arbitrary set (not necessarily even a
vector space); $I$ is the $d \times d$ identity matrix; $f:\mathcal{X}
\times \mathcal{U}\rightarrow
\mathcal{X}$; and  where $t\in [H]$ with $[H] = \{1, 2, \ldots
H\}$. 
 Throughout, we assume that $x_0$ is a fixed starting state. 

A controller is a mapping $\pi: \mathcal{X}\times \{0,\ldots H-1\} \rightarrow
\mathcal{U}$.   Given a instantaneous cost function $c:\mathcal{X} \times
\mathcal{U}\rightarrow \R$, we define the cost (or the ``cost-to-go'' ) of a policy as:
\[
J^\pi(x;c) =  \Exp \left[ \sum_{h=0}^{H-1} c(x_h, u_h)  \Big|
  \pi, x_1=x
\right] 
\label{eq: cost}
\]
where the expectation is under trajectories sampled under $\pi$ starting from $x_0$.
The cost at state $x$ at time $\tau$ is denoted by:
\[
J^\pi_\tau(x;c)  = \Exp \left[ \sum_{h=\tau}^{H-1} c(x_h, u_h)  \Big|
  \pi, x_\tau=x
\right]  \, .
\]
The ``state-control cost'' at state $x$ and taking control $u$ at time $\tau$ and then
following $\pi$ is denoted by:
\[
J^\pi_\tau(x,u;c)  = \Exp \left[ \sum_{h=\tau}^{H-1} c(x_h, u_h)  \Big|
  \pi, x_\tau=x, u_\tau=u
\right]  \, .
\]
We will assume that these expectations exist for all policies
$\pi\in\Pi$ throughout. %\akshay{Two comments here: Is $\Pi$ defined? And is this assumption reasonable with unbounded costs?} 
\fi

\iffalse
Given some class of policies $\Pi$, we will denote the optimal cost
and optimal state-control cost as:
\[
J^\star_\tau(x;c)  = \min_{\pi\in\Pi} J^\pi_\tau(x;c) , \ \textrm{ and } \ 
J^\star_\tau(x,u;c)  = \min_{\pi\in\Pi} J^\pi_\tau(x,u;c)
\]
Note that optimality here is defined with respect to the policy class $\Pi$.
\fi

\iffalse
Consider the problem of sequentially optimizing a 
sequence of cost functions where the nonlinear dynamics $f$ are unknown.
In each episode $t$, we observe an instantaneous cost function $c^t$; we
choose a policy $\pi^t$; we execute $\pi^t$ and observe a sampled trajectory $x_0,u_0, \ldots
x_H,u_H$; we incur the cumulative cost:
\[
\widehat J^t = \sum_{h=0}^{H-1} c^t(x_h, u_h)  \, .
\]
Our goal is to minimize the sum
of our costs over $T$ rounds. In particular, we desire to execute a policy
that is nearly optimal for every episode.

A natural performance metric in this context is cumulative regret, the
increase in cost due to not knowing the nonlinear dynamics
beforehand. The instantaneous regret at the $t$-th episode is defined as:
\[
\widehat J^t - \min_{\pi\in\Pi} J^\pi(x_0;c^t)
\]
and the cumulative regret over $T$ rounds is defined as:
\[
\textsc{Regret}_T =  \sum_{t=0} ^{T-1} \widehat J^ t - \sum_{t=0} ^{T-1} \min_{\pi\in\Pi} J^\pi(x_0;c^t)
\]
A desirable asymptotic property of an algorithm is to be no-regret, i.e.
$\lim_{T\rightarrow\infty}\textsc{Regret}_T / T =0$. 

\paragraph{GP priors.} 
Here, we assume that $f \sim GP(0,K( x,u; x',u' ) )$ for some known
kernel $\mathbf{k}$.
We assume the kernel $\mathbf{k}$ as the following property.  

\begin{asm} \sk{do we need this assumption?} For a sampled path $f\sim GP$, there exist constants $a\in \mathbb{R}^+$ and $b\in\mathbb{R}^+$, such that:
\begin{align*}
\mathrm{Pr}\left( \forall z,i, |\partial f / \partial z_i| > L\right) \leq a\exp(-(L/b)^2).
\end{align*}
\end{asm}
\fi

\paragraph{$f$ in the RKHS.}
In a more agnostic sense, we can alternatively assume that $f$ lives
in the RKHS of a known kernel $K$. Equivalently, the primal version of
this assumption is that:
\[
f(x,u) = W \phi(x,u)
\]
for some known function $\phi: \mathcal{X}\times\mathcal{U}
\rightarrow \mathcal{V}$ where $\mathcal{V}$ is either a finite or
countably infinite dimensional Euclidean vector space and where $W$ is
a linear mapping.

\begin{asm} Given a cost function $c$ and a model $f$, we have an
  optimal planner $\pi = \textsc{Plan}(c, f)$ that outputs the best
  policy over a policy set, i.e., $\pi = \arg\min_{\pi\in\Pi}
  J^{\pi}(c, f)$. \sk{need to assume LCB planner}
\end{asm}

\iffalse
\begin{asm}\label{asm:bounded_cost} We assume the total realize cost, $\sum_{h=0}^{H-1} c^t(x_h,
  u_h) $  is bounded by $J_{\max}$, i.e., for any $c^t$ and any policy $\pi\in\Pi$.
% $W$ has bounded norm $\|W\|_F \leq \sqrt{d} u$, and $\phi$ has bounded norm, i.e., $\sup_{z}\|\phi(z)\|_2 \leq 1$.
\end{asm}
\fi

\paragraph{Linear Quadratic Regulators (LQR) as a special case}
Our model generalizes Linear Quadratic Regulator (LQR). Specifically,
we can set $\phi(x,u) = [x^{\top}, u^{\top}]^{\top}$, $c(x,u) =
x^{\top} Q x + u^{\top}R u$ with $Q$ and $R$ being some PSD matrix.
The policy class in this case will be all linear controls, i.e., $\Pi
= \{\pi: u = Kx, K\in\mathbb{R}^{d_{u}\times d_{\calX}}\}$. 



\paragraph{Notation.} \sk{some of this should go into the appendix}
Unless otherwise specified, subscripts refer to
the timestep within an episode and superscripts index the episode
itself, i.e. $\phi^t_h$ will refer to the random vector which is the
observed features during timestep $h$ within episode $t$.  We let
$\mathcal{H}^t_h$ denote the history of all observations before
the $h$-th timestep in episode $t$. 
%We slightly abuse note and use $\mathcal{H}^t_h$ to also denote the
%index set of all pairs of timesteps and episodes observed before the
%$h$-th timestep in episode $t$. 

We implicitly drop the policy dependence when clear from context,
e.g. we write $J^{t}(x;c)$ instead of $J^{\pi^t}(x,c)$ 
%\akshay{This could be confusing. $J^t$ is already defined as the realized cost of the algorithm on episode $t$. Is $J^{\pi^t}$ the realized or the expected cost?}.
We use the notation $J^\pi(x;c,W) $ to be the cost function under
model $W$. 
%Due to that $x_0$ is our fixed starting state, for notational
%convenience, we sometimes write $J^\pi(c)$ and $J^\pi(c,W)$ instead of
%$J^\pi(x_0;c)$ and $J^\pi(x_0;c,W)$ , when clear from context.

For a matrix $M$, we use $\|M\|_2$ and $\|M\|_F$ to denote the spectral
and Frobenius norms.
 
